UrbanVR: An immersive analytics system for context-aware urban design

Urban design is a highly visual discipline that requires visualization for informed decision making. However, traditional urban design tools are mostly limited to representations on 2D displays that lack intuitive awareness. The popularity of head-mounted displays (HMDs) promotes a promising alternative with consumer-grade 3D displays. We introduce UrbanVR, an immersive analytics system with effective visualization and interaction techniques, to enable architects to assess designs in a virtual reality (VR) environment. Specifically, UrbanVR incorporates 1) a customized parallel coordinates plot (PCP) design to facilitate quantitative assessment of high-dimensional design metrics, 2) a series of egocentric interactions, including gesture interactions and handle-bar metaphors, to facilitate user interactions, and 3) a viewpoint optimization algorithm to help users explore both the PCP for quantitative analysis, and objects of interest for context awareness. Effectiveness and feasibility of the system are validated through quantitative user studies and qualitative expert feedbacks.

==> discussion.tex <==
\section{Discussion}	\label{sec:dis}
Currently, limited interactions of building manipulation and map navigation are supported by Ur-banVR. More advanced interactions for exploring analysis results, such as to filter and reconfigure the PCP~\cite{4376144}, are missing. This limits analysis functionality of our system. For instance, the collabo-rating architect would like our system to filter and sort designs according to a specific criteria. UrbanVR will be more useful if such features are integrated. A main obstacle is that the raw gesture detection provided by Leap Motion is not accurate enough. We look forward to more advanced gesture detection devices in the near future. With more accurate and robust gesture interactions, we can further improve the interface design, following the guidelines for interface design for virtual reality~\cite{BOWMAN199937}.

For the moment, we integrate viewpoint optimization and handle bar metaphor to improve gesture interactions. The user study shows that handle bar (C3), and handle bar + viewpoint optimization (C4) facilitate gesture interaction in terms of completion time. The tasks require users to match a building’s position, size, and orientation with a target building. Hence, the matching can also be considered as an accuracy test. In terms of this, the handle bar also improves the accuracy of ges-ture interactions. However, results for viewpoint optimization as a supplement to gesture interac-tions (C2) do not distribute normally. This may be because the participants are not familiar with viewpoint optimization. More try-outs may suppress the participant’s cognitive bias on viewpoint optimization. Another reason can be the optimal viewpoint may not be ‘true’ optimal due to the LOD simplification method employed in this work. A sophisticated evaluation will be carried out to improve the method~\cite{10.1145/3209661}. Nevertheless, feedbacks from the participants and domain experts suggest that viewpoint optimization is helpful and necessary.

Besides viewpoint optimization, another popular occlusion minimization and view enhancement method is $focus + context$, which has also been well-studied in the visualization and graphics communities. Recently, some study has applied this method to urban scenes~\cite{7208899}. The method allows buildings to be shifted and scaled, thus should generate views with less occlusion than our approach. However, the distortion of urban scene can increase users’ mental mapping of reality in the virtual world. Considering the benefits and drawbacks, it is worth another study to compare the effectiveness of these methods for immersive analytics.
